FLToP CTC: Frame-Level Token Pruning via Relative Threshold for Efficient and Memory-Saving Decoding on Diverse Platforms

CTC-based ASR systems face computational and memory bottlenecks in resource-limited environments. Traditional CTC decoders, requiring up to 90% of processing time in systems (e.g., wav2vec2-large on L4 GPUs), face inefficiencies due to exhaustive token-level operations. This paper introduces Frame Level Token Pruning for Connectionist Temporal Classification (FLToP CTC), a novel decoding algorithm that employs frame-level token pruning guided by a relative threshold probability. By dynamically eliminating low-probability tokens per frame, FLToP CTC reduces compute and memory demands while maintaining negligible WER degradation. On LibriSpeech, FLToP CTC achieves a 10.5x runtime speedup and 2.78x memory reduction versus standard CTC decoders. Its simplicity enables seamless integration into CTC decoders across platforms (CPUs, GPUs, etc.). FLToP CTC addresses CTC bottlenecks, offering scalability for resource-limited environments and realtime applications, enhancing speech recognition accessibility and efficiency.

==> section/results.tex <==
\section{Results}\label{sec:results}
%This section provides a detailed results and analysis of all the experiments we conducted to see the impact of the newly added parameter relative\_token\_threshold from our new novel approach for Frame Level Relative Token Pruning. This is to show how the new approach improve the computational efficiency.

\subsection{Index tracking of Chosen Token}
\label{subsec:results_index_track_chosen_token}
% \noindent\textbf{Index tracking of Chosen Token:} 
We examineedsw the distribution of selected tokens by charting the frequency with which tokens at certain sorted index positions are chosen, analyzing this across the entire dataset and all timesteps. Figure~\ref{fig:resultsindex_counts_stats_sortedTokenProbs_batchsize32_softmax_numHyps_tokenSize32_tokenRel_0.0} demonstrates that tokens at lower indices, closer to index 0, are selected more frequently because they have higher emission scores. Notably, indices such as 22, 27, and those beyond 28 do not appear in the plot, which means no tokens at these positions were chosen throughout the evaluation across all timesteps. Significantly, the frequency of selecting tokens past the fourth index is minimal, with $99.9823\%$ of token selections involving only up to the fourth index, and less than $0.0178\%$ involving tokens at higher indices. This data supports the strategy of retaining only the top-4 tokens and pruning others from the fifth index onwards. Furthermore, the plot in Figure~\ref{fig:resultsindex_counts_stats_sortedTokenProbs_batchsize32_softmax_numHyps_tokenSize32_tokenRel_0.0} also shows the average emission scores of tokens at each index, confirming that the tokens at lower indices consistently has a significantly higher score than any other token.

\noindent Key observations include:
\begin{itemize}[nosep,noitemsep,leftmargin=*]
    \item The counts scale is logarithmic. Even on a logarithmic scale, frequency appears to decrease exponentially with increasing index.
    \item Similarly, the emission score decreases exponentially as the index increases.
    \item Beam search aims for the highest joint probability, indicating that a candidate with a high beam score may still choose a token from a lower index during a particular timestep. This phenomenon is noticeable at far indices such as 16, 19, 21, 23, and others.
\end{itemize}



% \begin{table}[t]
%     \centering
%     \small
%      \caption{Token Statistics: Probability, Count, Cumulative Count, and Coverage}
%      \vspace{-4mm}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{ccccc}
%         \toprule
%         \textbf{Token Index} & \textbf{Avg. Probability} & \textbf{Index Count} & \textbf{Cumulative Count} & \textbf{Cumulative Ratio} \\
%         \midrule
%         0  & 70.62   & 1123786  & 1123786  & 0.9947  \\
%         1  & 8.708   & 4808     & 1128594  & 0.9989  \\
%         2  & 6.038   & 682      & 1129276  & 0.9996  \\
%         3  & 4.509   & 203      & 1129479  & 0.9997  \\
%         4  & 2.87    & 100      & 1129579  & 0.9998  \\
%         5  & 2.007   & 45       & 1129624  & 0.9999  \\
%         6  & 1.042   & 33       & 1129657  & 0.9999  \\
%         7  & 0.666   & 23       & 1129680  & 0.9999  \\
%         8  & 0.238   & 20       & 1129700  & 0.9999  \\
%         9  & -0.222  & 19       & 1129719  & 0.9999  \\
%         10 & -0.496  & 13       & 1129732  & 0.9999  \\
%         11 & -0.656  & 6        & 1129738  & 0.9999  \\
%         12 & -0.975  & 6        & 1129744  & 0.9999  \\
%         13 & -1.283  & 4        & 1129748  & 0.9999  \\
%         14 & -1.971  & 4        & 1129752  & 0.9999  \\
%         15 & -0.941  & 4        & 1129756  & 0.9999  \\
%         16 & -1.753  & 8        & 1129764  & 0.9999  \\
%         17 & -1.707  & 2        & 1129766  & 0.9999  \\
%         18 & -2.444  & 1        & 1129767  & 0.9999  \\
%         19 & -1.639  & 3        & 1129770  & 0.9999  \\
%         20 & -2.824  & 1        & 1129771  & 0.9999  \\
%         21 & -2.21   & 2        & 1129773  & 0.9999  \\
%         23 & -3.950  & 3        & 1129776  & 0.9999  \\
%         24 & -3.365  & 1        & 1129777  & 1.0000  \\
%         25 & -2.327  & 1        & 1129778  & 1.0000  \\
%         26 & -5.427  & 1        & 1129779  & 1.0000  \\
%         28 & -5.708  & 1        & 1129780  & 1.0000  \\
%         \bottomrule
%     \end{tabular}}
%     \vspace{-4mm}
%     \label{tab:token_stats}
% \end{table}

\subsection{Top-N thresholding for N = 1 \ldots 32 tokens} \label{subsec:results_exp_top_1_to_32}
% \noindent\textbf{Top-N thresholding for N = 1 \ldots 32 tokens:}
Figure~\ref{fig:wer_vs_decoding_time_relTokThres0.0_varyNumTokens_side_by_side_scatter} demonstrates how WER correlates with beam-size-tokens. Observational data indicates that any increase in tokens beyond Top-4 yields minimal reduction in WER; in fact, WER tends to rise marginally as the number of beam-size-tokens increases. Notably, limiting the search to Top-4 tokens results in a WER of 3.852, surpassing the baseline's exhaustive search (Top-32, WER = 3.864). Additionally, decoding time almost linearly increases with the number of beam-size-tokens. The baseline setting (Top-32) experiences a decoding time that is 3.94× longer than the Top-4 configuration, without any WER benefits. These results strongly support the use of Top-4 tokens as an efficient balance between accuracy and computational demands.

Based on these findings, we set N=4 for subsequent experiments to further enhance WER while minimizing computational costs. Reducing processing time is essential for implementing models in real-time applications with limited resources. This leads us to develop a novel strategy aimed at boosting decoding efficiency without compromising the accuracy of transcription.


\subsection{Relative Token Thresholding (N = 4, R varying):}
\label{subsec:results_rel_token_thres_top4}
% \noindent\textbf{Relative Token Thresholding (N = 4, R varying):}
Figure~\ref{fig:wer_vs_decoding_time_top4_varyRelTokThres_side_by_side_scatter} displays the impact of adjusting the $R$ parameter in Algorithm~\ref{algo:beam_search_fltop_ctc_decoding_for_asr} on both decoding time and WER. A notable decrease in decoding time is observed when using this method compared to the Top-4 approach, without any loss in transcription accuracy. Specifically, setting $R = 0.007$ reduces the decoding time to 369.6 seconds, achieving a speed~$2.78\times$ faster than the Top-4 method and~$10.5\times$ faster than the baseline. Furthermore, WER slightly improves to 3.843 from 3.852, which is seen in the Top-4 method without relative pruning. The optimal WER recorded is 3.831 at $R= 0.001$, which processes faster than using Top-4 pruning alone, although it is marginally slower than at the 0.007 threshold due to reduced pruning.

These results validate the efficacy of frame-level token pruning based on the highest token’s emission score. Despite the wide range of $R$ from $0.5$ to $0.003$, which adjusts the pruning effect significantly (allowing tokens whose emission score is at least 50\% to 0.3\% of the top token's score), the time differences between these extreme values are minimal. Typically, only 1 to 2 tokens from the top 4 are selected for beam search with both $0.5$ and $0.003$ as $R$ values. However, with larger vocabularies and higher Top-N settings, the benefits of relative token pruning become more evident. With more tokens eligible for pruning, significant improvements in decoding speed can be achieved, especially when the encoder outputs are highly confident. When emission scores are more evenly distributed across tokens, varying $R$ affects decoding performance more substantially.

\subsection{Relative Token Thresholding impact on Number of Beams and Memory Consumption} \label{subsec:results_rel_tok_impact_on_memory}
% \noindent \textbf{Relative Token Thresholding impact on Number of Beams and Memory Consumption:}
Figure~\ref{fig:results_hypothesis_stats_top4_relTokThres0.007} displays a box plot depicting the distribution of beam counts maintained throughout all timesteps within the dataset. The Interquartile Range (IQR) distinctly shows that our method requires fewer beams compared to other methods, while still preserving ASR performance, underscoring the efficiency of frame-level relative pruning. Typically, our model maintains only 2 beams for the majority of timesteps, which reflects substantial improvements in both computational and memory efficiency. On average, our approach maintains 214.4 beams, whereas the baseline configuration and the Top-N pruning (N=4) method maintain 596.26 beams (2.78 times more) and 461.99 beams (2.15 times more), respectively. The box plot further highlights that the mean, median, and quartiles for beam counts in our method are consistently lower than those in the baseline and Top-N configurations, affirming that FLToP CTC (Frame-Level Token Pruning CTC) surpasses conventional approaches in memory efficiency and aligns with previous WER findings.


%\subsection{Tips to fine-tune the relative\_token\_threshold parameter}\label{subsec:results_tune_rel_token_thres}
% \noindent\textbf{Tips to fine-tune the relative\_token\_threshold parameter}
% From the Fig.  \ref{fig:resultsindex_counts_stats_sortedTokenProbs_batchsize32_softmax_numHyps_tokenSize32_tokenRel_0.0}, we can find that most of the time we chose only those tokens in the indexes near to 0 after sorting. So we can make use of the average emissions scores of all those tokens occurring at same index after sorting and can chose the relative\_token\_threshold parameter based on the token choosing coverage threshold we expect to happen (by making use of the information about count of choosing each index across whole dataset) to know till how many tokens needs to be allowed based on the average scores of each token. Table \ref{tab:token_stats} shows how to set the relative\_token\_threshold parameter based on the token coverage threshold. For instance, if you want to cover 99.99\% of tokens to be correctly chosen (approximately), then we need to allow till token index 5 whose average probability is 2.007. So the relative\_token\_threshold values should be 2.007/70.62 which is 0.028419. So based on the token count ration, we can map the desired coverage count with the relative\_token\_threshold value. Note that when dealing negative values, it is recommended to normalize the average probabilities and then find the relative\_token\_threshold value. If the average probability values are not strictly decreasing then need to use the cumulative summation approach for finding the right relative\_token\_threshold. 
